TMAC: A Toolbox of Modern Async-Parallel, Coordinate, Splitting, and Stochastic Methods

TMAC is a toolbox written in C++11 that implements algorithms based on a set of modern methods for large-scale optimization. It covers a variety of optimization problems, which can be both smooth and nonsmooth, convex and nonconvex, as well as constrained and unconstrained. The algorithms implemented in TMAC, such as the coordinate up- date method and operator splitting method, are scalable as they decompose a problem into simple subproblems. These algorithms can run in a multi-threaded fashion, either synchronously or asynchronously, to take advantages of all the cores available. TMAC architecture mimics how a scientist writes down an optimization algorithm. Therefore, it is easy for one to obtain a new algorithm by making simple modifications such as adding a new operator and adding a new splitting, while maintaining the multicore parallelism and other features. The package is available at https://github.com/uclaopt/TMAC.

==> documentation.tex <==
% !TEX root = ./arock_pkg_main.tex
\subsection{Documentation}
\begin{itemize}
\item html docs;
\item heavily commented code; 
\item example code;
\item youtube HOWTO;
\end{itemize}


==> fpp.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{The Fixed-point Problem}
\begin{enumerate}
\item the fixed-point problem;
\item cached variables;
\item and refer everything else to CF-paper;
\end{enumerate}


==> huber_loss.tex <==
% !TEX root = ./arock_pkg_main.tex
\subsection{Minimizing Huber Loss}
Might delete this.

==> installation.tex <==
% !TEX root = ./arock_pkg_main.tex
\subsection{Practical Usage}
\begin{itemize}
\item download;
\item script for downloading the required packages; 
\item script to do prepackage solvers;
\end{itemize}



==> organization.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{Organization}
\begin{enumerate}
\item Introduction
\item The fixed-point problem
\item The software package
	\begin{enumerate}
	\item Practical usage;
	\item Documentation;
	\item Design;
	\end{enumerate}
\item Comparison;

\item Conclusion 

\item Appendix (derivation of the examples??)

\end{enumerate}


==> quick_start.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{Quick Start}\label{sec:quick_start}
 To illustrate the practical usage of ARock, we use the $\ell_1$ regularized logistic regression
\begin{equation}\label{eq:l1_log}
\min_{x \in \RR^n} \lambda \|x\|_1 + \sum_{i = 1}^m \log\left(1 + \exp(-b_i \cdot a_i^T x)\right)
\end{equation}
as an example, where $\{(a_i, b_i)\}_{i = 1}^m$ is the training dataset. We set the regularization parameter $\lambda$ to 1, and set the maximum number of epochs to 10. The following is the command to train the model on the news20\footnote{ This dataset is from \url{http://www.csie.ntu.edu.tw/~cjlin/libsvmtools/datasets}.} dataset with 2 threads,
\begin{lstlisting}[language=bash]
$ arock_fbs_l1_log -data news20.svm -epoch 10 -nthread 2 -lambda 1.
[other outputs skipped]
Computing time  is: 4.88(s).
\end{lstlisting}
where \texttt{-data, -epoch, -nthread, -lambda} are the flags for the data file, maximum number of epochs, total number of threads, and regularization parameter $\lambda$ respectively. We can see that the command-line tool is easy-to-use. Beyond the simplicity, ARock is also efficient in the sense that the training time is less than 5 seconds for a problem with more than 1 million variables. Next, we show the major components of the source codes for building \texttt{arock\_fbs\_l1\_log}.

We solve \eqref{eq:l1_log} with the forward-backward splitting scheme
\begin{equation}\label{eq:fbs_l1_log}
x^{k+1} = \underbrace{\prox_{\lambda \eta \|x\|_1}}_{\text{backward operator}} (\underbrace{x^k - \eta \, \nabla \,\sum_{i = 1}^m \log (1 + \exp(-b_i \cdot a_i^T x^k)}_{\text{forward operator}}),
\end{equation}  
where the gradient step of logistic loss and the proximal operator of $\ell_1$ norm correspond to the forward step and backward step respectively. The following snippet of code (extracted from \texttt{apps/arock\_fbs\_l1\_log.cc}) implements \eqref{eq:fbs_l1_log} with the ARock framework. Specifically, line 2 and line 5 define the forward operator and backward operator respectively. Line 3 and line 6 use \texttt{decltype} to simplify the names for the operator types. Line 7 define the FBS with the previously defined forward and backward operators. Line 8 calls \texttt{AROCK} on the \texttt{fbs}  object. We can see that creating an async-parallel solver can be easily achieved through assembling appropriate operators together.  
\begin{lstlisting}[language=C++]
  // forward operator: gradient step for logistic loss
  forward_grad_for_log_loss<SpMat> forward(&A, &b, &Atx, eta);
  using F = decltype(forward); // yields the type of forward
  // backward operator: proximal operator for l1 norm 
  prox_l1 backward(eta, lambda);
  using B = decltype(backward); // yields the type of backward
  ForwardBackwardSplitting<F, B> fbs(&x, forward, backward);  
  AROCK(fbs, params);  
\end{lstlisting}

==> related_work.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{Related Works}
\begin{enumerate}
\item review existing for serial implementation and theory of CU method (steel some from the CF paper);
\item review existing sync-parallel solvers, so far we are aware of the followings 
\begin{itemize}
\item ac-dc package: \url{https://github.com/optml/ac-dc}, 
\end{itemize}
\item review existing async-parallel solver:
\begin{itemize}
\item Passcode: \url{http://www.cs.utexas.edu/~rofuyu/exp-codes/passcode-icml15-exp/}
\item Hogwild: \url{http://i.stanford.edu/hazy/victor/Hogwild/}
\end{itemize}

\end{enumerate}


==> software.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{The Software Package}

\input{installation}

\input{documentation}

\input{architecture}

==> syntax.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{Syntax}



==> system_intro.tex <==
% !TEX root = ./main.tex
\section{Overview of Multi-core Computer Systems}
A multi-core computer system uses two or more cores. The system can have multiple chips or multiple cores on a single chip. There are two major types of multi-core systems: shared-memory systems and distributed memory systems. In this thesis, we will discuss the realizations of CU methods on both shared memory system and distributed memory systems. 

\subsection{Shared Memory Systems}
In shared memory systems, multiple processors are connected to a memory system via an interconnection network, and each processor can access each memory location. These processors usually communicate with each other implicitly through shared data structures. Depending on the type of interconnect, shared memory systems can be classified into two types: uniform memory access (UMA) system and nonuniform memory access (NUMA) system. UMA system connects all the processors directly to main memory. All processors in NUMA system have a direct connect to a block of main memory and they can access each others' blocks memory through hardware built into the processors. Figure~\ref{fig:shared_mem} shows the architectures for the two types of shared memory systems.\footnote{The figure is adapted from Figure 2.5 and Figure 2.6 in \cite{pacheco2011introduction}.} 
\begin{figure}[!h]
        \centering
       \begin{subfigure}[b]{0.45\textwidth}
                \includegraphics[width=\textwidth]{./figs/uma.eps}
                \caption{UMA system.}\label{fig:consist}
        \end{subfigure}
        ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
          %(or a blank line to force the subfigure onto a new line)
        \begin{subfigure}[b]{0.45\textwidth}
                \includegraphics[width=\textwidth]{./figs/numa.eps}
                \caption{NUMA system.}\label{fig:inconsist}
        \end{subfigure}
        \vspace{-3mm}
        \caption{Architectures for UMA and NUMA systems.}
        \vspace{-3mm}
        \label{fig:shared_mem}
\end{figure}


\subsection{Distributed Memory Systems}
Distributed memory system consists of a collection of commodity processors which are connected by a interconnection network. Each processor has its own private memory and communicates others by explicitly sending messages through an interconnection network. Figure~\ref{fig:dist_sys} demonstrates the architecture for distributed memory systems.  
\begin{figure}[!h]
      \centering
        \includegraphics[width=0.5\textwidth]{./figs/distributed_sys.eps}
      \caption{Architectures for distributed memory systems.}
        \label{fig:dist_sys}
\end{figure}




==> user_interaction.tex <==
% !TEX root = ./arock_pkg_main.tex
\section{User Interaction}

\begin{itemize}
\item Implement apps (using library);
\item Using synchronous;
\item Implement your own operator;
\item implement your own coordinate update (put the entire update to a single operator)
\end{itemize}

